Pick Planning Strategies for Large-Scale Package Manipulation

Automating warehouse operations can reduce logistics overhead costs, ultimately driving down the final price for consumers, increasing the speed of delivery, and enhancing the resiliency to market fluctuations. This extended abstract showcases a large-scale package manipulation from unstructured piles in Amazon Robotics' Robot Induction (Robin) fleet, which is used for picking and singulating up to 6 million packages per day and so far has manipulated over 2 billion packages. It describes the various heuristic methods developed over time and their successor, which utilizes a pick success predictor trained on real production data. To the best of the authors' knowledge, this work is the first large-scale deployment of learned pick quality estimation methods in a real production system.

==> figures_tikz/layers/block-diagram.tex <==
\usetikzlibrary{shapes,arrows,shadows,fadings}
\usetikzlibrary{positioning}

% ------------------------------------- Color Definitions -------------------------------------------------------
\colorlet{BlockFillColor}{JungleGreen!40}
\colorlet{BlockBorderColor}{JungleGreen!70}
\colorlet{RobotColor}{cyan!20}
\colorlet{NewModuleFillColor}{Violet!20}
\colorlet{NewModuleBorderColor}{Violet!70}
\colorlet{BackgroundModuleBorderColor}{Magenta!70}
\colorlet{BackgroundModuleFillColor}{Lavender!20}
\colorlet{ModifiedModuleBorderColor}{RedOrange!70}
\colorlet{ModifiedModuleFillColor}{Peach!20}


% ------------------------------------- Block Definitions -------------------------------------------------------

\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{shadowstyle} = [drop shadow={top color=gray, bottom color=white, shadow xshift=\picscale*0.8mm, shadow yshift=-\picscale*0.8mm, rounded corners=\picscale*1mm}]

\tikzstyle{block} = [draw=BlockBorderColor, shadowstyle, fill=BlockFillColor, shape=rectangle, rounded corners=\picscale*1mm, minimum height=\picscale*5em, minimum width=\picscale*11.5em, align=center, node distance=\picscale*4cm]
%\tikzstyle{sum} = [draw, fill=BlockColor, circle, node distance=\picscale*1cm]
\tikzstyle{input} = []
\tikzstyle{optinput} = [input, draw, rectangle, densely dashed, inner sep=\picscale*0.5pt]
\tikzstyle{output} = [block, fill=RobotColor, node distance=\picscale*2.5cm]
\tikzstyle{feedback} = [coordinate, node distance=\picscale*2cm]
\tikzstyle{joint} = [coordinate]

\tikzstyle{newmodule} = [block, fill=NewModuleFillColor, draw=NewModuleBorderColor]
\tikzstyle{modifiedmodule} = [block, fill=ModifiedModuleFillColor, draw=ModifiedModuleBorderColor]

\tikzstyle{sum} = [draw=BlockBorderColor, shadowstyle, fill=BlockFillColor, circle, minimum size=\picscale*1cm, node distance=\picscale*1.75cm]

==> figures_tikz/layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}



==> preamble.tex <==
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{array}
\usepackage{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[subfigure]{labelformat=simple}
% \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{textcomp} % This package is also used for trademark symbol and proper tilde sign
\usepackage{stfloats}
\usepackage[hyphens]{url}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}
\usepackage[numbers]{natbib}
% \usepackage{cite}
% \hyphenation{op-tical net-works semi-conduc-tor IEEE-Xplore}
\usepackage{times}
% numbers option provides compact numerical references in the text. 
\usepackage{multicol}
% \usepackage[bookmarks=true]{hyperref}
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}

% Define the enumeration
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{tabularx}
% \renewcommand\labelitemi{---}

\usepackage{booktabs}       % professional-quality tables

% Allow dashed \midrule in the table
\usepackage{arydshln}
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother

% Update tilde ~ sign to look "normal" as it should!
\newcommand{\textmidtilde}{\raisebox{0.5ex}{\texttildelow}}

\newcommand{\nth}[1]{$#1^{\text{th}}$}

% % Define commenting
% \newcommand{\kevin}[1]{\textcolor{red}{KGJ: #1}}
% \newcommand{\azarakhsh}[1]{\textcolor{blue}{AK: #1}}
% \newcommand{\nick}[1]{\textcolor{cyan}{NH: #1}}
% \newcommand{\shuai}[1]{\textcolor{purple}{SL: #1}}
% \newcommand{\placeholder}[1]{\textcolor{Magenta}{#1}}

